Search-Based Regular Expression Inference on a GPU

Regular expression inference (REI) is a supervised machine learning and program synthesis problem that takes a cost metric for regular expressions, and positive and negative examples of strings as input. It outputs a regular expression that is precise (i.e., accepts all positive and rejects all negative examples), and minimal w.r.t. to the cost metric. We present a novel algorithm for REI over arbitrary alphabets that is enumerative and trades off time for space. Our main algorithmic idea is to implement the search space of regular expressions succinctly as a contiguous matrix of bitvectors. Collectively, the bitvectors represent, as characteristic sequences, all sub-languages of the infix-closure of the union of positive and negative examples. Mathematically, this is a semiring of (a variant of) formal power series. Infix-closure enables bottom-up compositional construction of larger from smaller regular expressions using the operations of our semiring. This minimises data movement and data-dependent branching, hence maximises data-parallelism. In addition, the infix-closure remains unchanged during the search, hence search can be staged: first pre-compute various expensive operations, and then run the compute intensive search process. We provide two C++ implementations, one for general purpose CPUs and one for Nvidia GPUs (using CUDA). We benchmark both on Google Colab Pro: the GPU implementation is on average over 1000x faster than the CPU implementation on the hardest benchmarks.

==> authorInfo.tex <==
\author{Mojtaba Valizadeh}
\email{Valizadeh.Mojtaba@gmail.com}
\orcid{https://orcid.org/0000-0003-1582-3213}
\affiliation{                                                                                                                                                                                                                                      \institution{University of Sussex}
  \city{Brighton}
  \country{UK}
}

\author{Martin Berger}
\email{contact@martinfriedrichberger.net}
\orcid{https://orcid.org/0000-0003-3239-5812}
\affiliation{   
  \institution{Montanarius Ltd}
  \city{London}
  \country{UK}
}
\affiliation{   
  \institution{Huawei R\&D UK Ltd}
  \city{London}  
  \country{UK}
}
\affiliation{                                                                                                                                                                                                                                      \institution{University of Sussex}
  \city{Brighton}
  \country{UK}
}





==> code/main_algorithm.tex <==
\begin{algorithm}
	
	\scriptsize
	\caption{Main function of synthesis algorithm}\label{algo_pseudo_main}
	
	\begin{algorithmic}[1]
		
		\State \textbf{Input} Positive and negative examples $\mathcal{(P, N)}$, \\ costFun [$c_1$, $c_2$, $c_3$, $c_4$, $c_5$], $maxCost$
		\State \textbf{Output} A minimal RE w.r.t costFun and $maxCost$ \\ and consistent with $\mathcal{(P, N)}$, otherwise "not\_found"
		
		\\\hrulefill
		
		\If {$\mathcal{P} == \{\}$} \Return "Empty" \EndIf
		\If {$\mathcal{P} == \{""\}$} \Return "Epsilon" \EndIf
		
		\State initialisation(gt, $P_t$, $N_t$)
		
		\State cache = [list of REcs(s) of alphabet] \Comment{in level c1}
		
		\State $result$ = ""
		
		\For{$cost \gets c_1 + 1$ to $maxCost$}
		
			\State uniqueList = QuestionMark(cache[$cost - c_2$], $P_t$, $N_t$)
			\If {$result$ != ""} \Return $result$ \EndIf
			\State cache[$cost$].insert(uniqueList)
			
			\State uniqueList = Star(cache[$cost - c_3$], $P_t$, $N_t$)
			\If {$result$ != ""} \Return $result$ \EndIf
			\State cache[$cost$].insert(uniqueList)
			
			\For{$i \gets c_1$ to $(cost - c_4)  /  2$}
				\State uniqueList = Concat(cache[$i$], cache[$cost - c_4 - i$], $P_t$, $N_t$)
				\If {$result$ != ""} \Return $result$ \EndIf
				\State cache[$cost$].insert(uniqueList)
			\EndFor
			
			\For{$i \gets c_1$ to $(cost - c_5)  /  2$}
				\State uniqueList = Or(cache[$i$], cache[$cost - c_5 - i$], $P_t$, $N_t$)
				\If {$result$ != ""} \Return $result$ \EndIf
				\State cache[$cost$].insert(uniqueList)
			\EndFor
		
		\EndFor
		
		\State \Return "not\_found"
		
	\end{algorithmic}
\end{algorithm}


==> code/or.tex <==
\begin{algorithm}
	
	\scriptsize
	\caption{Pseudocode implementing the union operation}\label{algo_pseudo_or}
	
	\begin{algorithmic}[1]
		
		\State \textbf{Input} Available cost, globals used: \texttt{languageCache}, P, N
		\State \textbf{Output} A list of new REcs(s) generated by \textit{or}
		
		\\\hrulefill
		
		\State outList $\gets$ []
                \ForAll{l, r \text{such that} l+r = cost} \Comment{Parallel on GPU version}
		\ForAll{$lREcs \in languageCache(l)$} \Comment{Parallel on GPU version}
			\ForAll{$rREcs \in languageCache(r)$} \Comment{Parallel on GPU version}
				\State $newREcs \gets lREcs\ |\ rREcs$ \Comment{Bitwise or}
				\State $isUnique \gets$ hashSet.insert($newREcs$)
				\If{$isUnique$}
					\If{$newREcs \models (P, N)$}
						\State ... non-local exit, returning newREcs as RE 
					\EndIf
					\State outList.insert($newREcs$)
				\EndIf
			        \EndFor
		                \EndFor
                                \EndFor
		\State \Return outList
		
	\end{algorithmic}
\end{algorithm}


==> code/question_mark.tex <==
\begin{algorithm}
	
	\scriptsize
	\caption{Pseudocode implementing the at-most-once (aka QuestionMark)}\label{algo_pseudo_question}
	
	\begin{algorithmic}[1]
		
		\State \textbf{Input} A list of REcs(s) lst, REcs testers $P_t$ and $N_t$
		\State \textbf{Output} A list of new REcs(s) generated by \textit{question mark}
		
		\\\hrulefill
		
		\State outList $\gets$ []
		\ForAll{$REcs \in lst$} \Comment{Parallel on GPU version}
			\State $newREcs \gets REcs\ |\ 1$
			\State $isUnique \gets$ hashSet.insert($newREcs$)
			\If{$isUnique$}
				\If{$(newREcs\ \& \ P_t) == P_t$ {\bf and} $(\neg newREcs\ \& \ N_t) == N_t$}
					\State $result \gets$ toString(indexOf($newREcs$))
				\EndIf
				\State outList.insert($newREcs$)
			\EndIf
		\EndFor
		\State \Return outList
		
	\end{algorithmic}
\end{algorithm}


==> code/star.tex <==
\begin{algorithm}
	
	\scriptsize
	\caption{Pseudocode implementing Kleene-star}\label  {algo_pseudo_star}
	
	\begin{algorithmic}[1]
		
		\State \textbf{Input} A list of REcs(s) lst, guide table gt, REcs testers $P_t$ and $N_t$
		\State \textbf{Output} A list of new REcs(s) generated by \textit{star}
		
		\\\hrulefill
		
		\State outList $\gets$ []
		\ForAll{$REcs \in lst$} \Comment{Parallel on GPU version}
			\State $c \gets 1$
			\State $newREcs \gets REcs\ |\ 1$
			\For{$bitIdx \gets 1$ to $numberOfInfixes$}
				\ForAll{pair ($l$, $r$) $\in$ gt[$bitIdx$]}
					\If{$(newREcs\ \& \ l) \neq 0$ {\bf and} $(newREcs\ \& \ r) \neq 0$}
						\State $newREcs \gets newREcs\ | \ c$
					\EndIf
				\EndFor
				\State $c \gets c \ll 1$
			\EndFor
			\State $isUnique \gets$ hashSet.insert($newREcs$)
			\If{$isUnique$}
				\If{$(newREcs\ \& \ P_t) == P_t$ {\bf and} $(\neg newREcs\ \& \ N_t) == N_t$}
					\State $result \gets$  toString(indexOf($newREcs$))
				\EndIf
				\State outList.insert($newREcs$)
			\EndIf
		\EndFor
		\State \Return outList
		
	\end{algorithmic}
\end{algorithm}


==> pldi_style.tex <==
%%% The following is specific to PLDI '23 and the paper
%%% 'Search-Based Regular Expression Inference on a GPU'
%%% by Mojtaba Valizadeh and Martin Berger.
%%%
\setcopyright{rightsretained}
\acmPrice{}
\acmDOI{10.1145/3591274}
\acmYear{2023}
\copyrightyear{2023}
\acmSubmissionID{pldi23main-p331-p}
\acmJournal{PACMPL}
\acmVolume{7}
\acmNumber{PLDI}
\acmArticle{160}
\acmMonth{6}
\received{2022-11-10}
\received[accepted]{2023-03-31}


